Learning to Teach Fairness-aware Deep Multi-task Learning

Fairness-aware learning mainly focuses on single task learning (STL). The fairness implications of multi-task learning (MTL) have only recently been considered and a seminal approach has been proposed that considers the fairness-accuracy trade-off for each task and the performance trade-off among different tasks. Instead of a rigid fairness-accuracy trade-off formulation, we propose a flexible approach that learns how to be fair in a MTL setting by selecting which objective (accuracy or fairness) to optimize at each step. We introduce the L2T-FMT algorithm that is a teacher-student network trained collaboratively; the student learns to solve the fair MTL problem while the teacher instructs the student to learn from either accuracy or fairness, depending on what is harder to learn for each task. Moreover, this dynamic selection of which objective to use at each step for each task reduces the number of trade-off weights from 2T to T, where T is the number of tasks. Our experiments on three real datasets show that L2T-FMT improves on both fairness (12-19%) and accuracy (up to 2%) over state-of-the-art approaches.

==> algo.tex <==


%For the dynamic selection of the loss function, we employ RL. 
An overview of our \emph{Learn to Teach Fairness-aware MTL (L2T-FMT)} algorithm is shown in Figure~\ref{fig:l2t_arc}. It is a teacher-student network framework; the student network has to learn a fair-MTL model, using advice from the teacher regarding the choice of the loss function. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/L2T_Fair_architecture_joined.pdf}
    \caption{The L2T-FMT architecture. Steps are in order from bottom to top}
    \label{fig:l2t_arc}
\end{figure*}

The student, teacher models are trained together as seen in Algorithm~\ref{algo:l2t}.
The \emph{teacher network}  $\mathcal{Q}$ aims at each training round to select the best loss function for each task among the two available options: accuracy loss and fairness loss (line 2). The selected loss function is adopted by the student network $\mathcal{M}$ and is used for network update (line 3).
After the update, the \emph{student network} provides feedback to the \emph{teacher network} about the progress made in each of the tasks following the advice of the \emph{teacher} (line 4).
 Based on the feedback, the \emph{teacher} network updates itself (line 5).
 So the two networks are trained collaboratively; their functionality  is explained in the next sections, for student (Section~\ref{sec:studentNetwork}) and teacher (Section~\ref{sec:teacherNetwork}).
Before that, we introduce the dynamic loss selection among the accuracy and fairness loss function choices (Section~\ref{sec:dynamic}).


%\subsection{L2T-FMT Algorithm}
\begin{algorithm}[!htbp]
	\caption{The L2T-FMT algorithm}
	\label{algo:l2t}
		\KwInput{A MTL dataset $D\in U\times S \times Y$ (see Section~\ref{sec:preliminaries})}
	\KwInit{Initialize student model  $\mathcal{M}$  parameters: $\theta=\theta_{sh}\times \theta_1\times\cdots\times\theta_T$ and 
	task weights: $w_t=\frac{1}{T}$\\
	Initialise teacher model $\mathcal{Q}$: parameters- $\theta^Q=\theta^Q_{sh}\times \theta^Q_1\times\cdots\times\theta^Q_T$ and environment weights  $w^Q=\{w^Q_t=\frac{1}{T}\}$
	}
	\begin{algorithmic}[1]
	    \State \textbf{Until} convergence \textbf{do}
	    \State \phantom{abv} \small$d=\{\argmax\limits_{\alpha \in \{\mathcal{L}_t,\mathcal{F}_t\}}Q(\theta_t,\alpha), \forall t\}$\normalsize \tcp{teacher decides the best loss to learn for student upon seeing $\theta_t$}
        \State \phantom{abc} Call Algorithm~\ref{algo:stud} with input $(U,S,Y,d)$\tcp{Training $\mathcal{M}$}
        %EIRINI: What is W?
        %\State \phantom{abc} \textbf{for} $t=1,\cdots,T$ \textbf{do}
        \State \phantom{abc} Evaluate $R=\{[\mathcal{R}(\mathcal{L}_t), \mathcal{R}(\mathcal{F}_t)]~\forall t\}$ using Eq.~\ref{eq:reward} \tcp{generate feedback for the teacher}
        %\State \phantom{abc} \textbf{end for}
        \State \phantom{abc} Call Algorithm~\ref{algo:teach} with input $(\{\mathcal{M}(t)\}, \{\theta_t\},R, A)$ \tcp{Training $Q$}
	\end{algorithmic}%}
	\KwOutput{$\mathcal{M}$ with learned parameters $\theta=\theta_{sh}\times \theta_1\times\cdots\times\theta_T$}
\end{algorithm}

% Regarding the task-specific weights $w_t$, instead of selecting the weights via hyperparameter tuning and
% fixing them over the training process as in~\cite{MTLfairWang0BPCC21}, we dynamically tune them over training, as argued earlier (cf. Section~\ref{sec:mtl}). 
% \color{black}






%In \textit{MTA-F} algorithm proposed by \cite{MTLfairWang0BPCC21} we see that for a fair-MTL model a separate update strategy using only task exclusive labels (e.g for a task $t$ exclusive labels  $ex_t=\{y_i^t=1|\forall_{k\neq t} y_i^k\neq 1\}$) for the task specific layer, uses of the model's fairness capacity better. However, intuitively, in presence of large number of tasks ($T>>2$) there may exist a very few or no such task exclusive label ($|ex_t|\approx 0$). While $ex_t=\emptyset$ will have no gradient update for fairness, but when the size of the set of such labels  ($ex_t$) is very small, a gradient based on such limited examples to generalize over the data, may update the model wrongly. Intuitively thinking as the task specific layers being the most important to any task $t$, we use the complete fairness info from all the available training data labels.  


 %; the goal of the student netwokr is to learn a fair-MTL model 
 % as shown  in Algorithm~\ref{algo:l2t} and explained in the next sections.

%The goal of the \emph{student network} is to learn a fair-MTL model $\mathcal{M}$ (see Subsection~\ref{sec:studentNetwork}).

 
%We first introduce the empirical- and fairness- loss functions we employ (Section~\ref{sec:ourLosses}). 

%For the dynamic selection of the loss function, we formulate the problem as an RL problem and we use DQN to approximate the values of the different states. In particular, 
%\todo{In Algorithm 1, what are the omega weights? never introduced before}



%using the GradNorm (cf. Eq.~\ref{eq:grad_norm}) loss. 
%Moreover, in order to learn a fair and accurate model across all the tasks it is important to find a correct balance of the task-specific weights $w_t$, a problem that is aggravated when the number of learning tasks is high. 
%Thus, to overcome %the obstacle we employ 
%the GradNorm \cite{chen2018gradnorm} for gradient balancing. 
%In practise, this means that the contribution of each task is balanced over training to ensure optimal algorithm and dynamically tune the task weights using the gradient of the selected loss. 
%\color{gray}



\subsection{Dynamic Loss selection}\label{sec:dynamic}
The fair-MTL problem definition (cf. Eq.~\ref{eq:mtlfair_summed}) introduces the $\lambda_t$ parameters for combining accuracy and fairness losses for each task  and therefore, the number of parameters required to be learned is doubled from $T$ (for traditional MTL, cf. Eq.\ref{eq:mtl}) to $2T$ (for fairness-aware MTL, cf. Eq.~\ref{eq:mtlfair_summed})). 
%making the learning relying more on finding these optimal weights.
%The seminar work~\cite{MTLfairWang0BPCC21} used hyperparameter tuning over a validation set to set the parameters $w_t$ and $\lambda_t$.
In this work, we propose to get rid of the $\lambda$ dependency and rather \emph{learn to choose} \emph{at each training step} whether the accuracy loss ($\mathcal{L}_t$) or the fairness loss ($\mathcal{F}_t$) should be used to train the model on task $t$. Such an approach reduces the optimization problem of Eq.~\ref{eq:mtlfair_summed} to that of Eq.~\ref{eq:mtl}, which is well studied in the literature~\cite{chen2018gradnorm,multi-task_gnn_2021deep,ecml_mtl_2021vogue,2021mtl_survey}. 
Moreover, it also provides the flexibility to the learner to emphasise on the objective (accuracy or fairness) that is harder to learn for each task at each training step.

The transformed learning problem is formulated as:
\begin{equation}\label{eq:prob_form}
    \argmin_{\theta, m} \sum_t w_t (m) 
    \begin{cases}
    \mathcal{L}_t(\theta,U,m), \text{if task $t$ is trained for \emph{accuracy} in epoch $m$}\\
    \mathcal{F}_t(\theta,S,m), \text{if task $t$, is trained for \emph{fairness} in epoch $m$}
    \end{cases}
\end{equation}
where $m$ is the epoch\footnote{To note that the epoch information though specifically used in Eq.~\ref{eq:prob_form} to understand the temporal aspect of the selection, is valid for all the previous and following equations and is omitted for the rest of the paper for ease of reading.} number that sequences until model convergence. %$(m=1,2,\cdots)$
%\todo{In this equation should be $\theta$ as in eq 2 or $\thera_Q$ as in eq 5?}
%\todo{What is not shown here is that the choice about hte loss is taken at each training step}
\color{black}

The accuracy loss and fairness loss functions that we adopt in this work are provided hereafter:

%\subsubsection{Empirical loss definitions}
%\label{sec:ourLosses}
\input{ourLosses}


\subsection{Student Network}
\label{sec:studentNetwork}
\input{student}

\subsection{Teacher Network}
\label{sec:teacherNetwork}
\input{teacher}

==> expTaskExlusiveLabels.tex <==
\color{blue}
ARA-> ACS-PUMS: 0.87 ($16\%\downarrow$), CelebA-Gender: 0.65 ($33\%\downarrow$), CelebA-Age: 0.69 ($27\%\downarrow$)
AREO-> ACS-PUMS: 3.39 ($180\%\uparrow$), CelebA-Gender: 1.41 ($6\%\downarrow$), CelebA-Age: 5.61($269\%\uparrow$)\\
\color{black}

We have seen that \our~outperforms \textit{MTA-F}~\cite{MTLfairWang0BPCC21}, which uses task-exclusive labels to update the task-specific parameters ($\theta_t$) and the rest of the labels to update the shared parameters ($\theta_{sh}$).
\color{red}
A set of exclusive labels for any task $t$ can be defined as the
examples that are only positive (negative) for the task $t$ and negative (positive) for the other tasks:  $ex_t=\{y_i^t=y|\forall_{k\neq t} y_i^k\neq y\}$, for $y\in\{0,1\}$. 
For \our we dont utilize task-exclusive labels but rather we exploit all instances for the update. \color{black}
To investigate the impact of not using $ex_t$, we compare \our~
%(with cumulative fairness of models 1 : j,where j is the current boosting round) 
with a version that considers
task-specific labels.
For this version, called \our\textit{-ex}, we update the task specific parameters $\theta_t$ with fairness head loss $\mathcal{F}^{head}_t$ calculated using $ex_t$ and the shared parameters $\theta_{sh}$ with fairness shared loss $\mathcal{F}^{head}_t$ calculated using the non-exclusive labels $\notin \cup_t ex_t$, following~\cite{MTLfairWang0BPCC21}.

% \begin{figure}[httb]
%     \centering
%     \begin{subfigure}[b]{0.45\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{Figures/box/ex_fair.png}
%          \caption{Boxplot fairness}\label{fig:box_ex_fair}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.45\columnwidth}
%          \centering
%          \includegraphics[width=\linewidth]{Figures/box/ex_acc.png}
%          \caption{Boxplot accuracy}\label{fig:box_ex_acc}
%     \end{subfigure}
%     \caption{\our vs \our\textit{-ex} trained on task-exclusive labels.}\label{fig:boxplot_ex}
% \end{figure}


% The results for the different datasets are shown in Fig.~\ref{fig:bfor the different datasets oxplot_ex}. 
% As can be seen, for the ACS-PUMS dataset with $T=5$ tasks, the performances are very close, esp. in fairness; for accuracy, \our~with non-exclusive labels performs better.
% But as the number of tasks increases (T=17 for CelebA-Gender and T=31 for CelebA-Age), the performance differences increase esp. w.r.t accuracy. \todo{How do you evaluate the differences thus far? It would also help to add the ARA AREO for this method too}

% %We see the difference is mainly attributed by 
% Moreover, there is an increase in spread of performance for \our\textit{-ex} which indicates the inconsistent performance of the method across different tasks. For some tasks the fairness performance is pretty bad (high upper whisker) and likewise for the accuracy (low lower whisker).
% %This shows that in some of the tasks \our\textit{-ex} performs very poorly in comparison to \our. 
% To gain insights on the results, we analyse the number of exclusive labels that are used to  update the task-specific parameters.
% For \emph{ACS-PUMS}, there is only 1 task (task 4) with very few exclusive labels (\#132), for the rest of the tasks, the number of exclusive labels is pretty high ($\geq 1.9K$). 
% \todo{I cannot see this in the figure.}Thus, we see in Fig~\ref{fig:box_ex_acc} that apart from only one task \our\textit{-ex} have high accuracy ($>0.60$) with low EO$_{viol}$ ($\leq0.04$).

% In \emph{CelebA-Gender} however, the total number of exclusive labels is very low ($ex_t\leq 806$) and 13 out of 17 tasks have less than 100 $ex_t$.
% For \emph{CelebA-Age} the situation is even worse as 29 out of 31 tasks have very few exclusive labels $(\leq 5)$. \todo{is the total number of exclusive labels again <806?} 
% \todo{Add smt here about what this means in terms of training. DO I recall correctly that the exclusive labels where used for fairness tuning?}

% This in turn effects the performance of \our\textit{-ex} resulting in low accuracy (on both CelebA-Gender and CelebA-Age) and high EO$_{viol}$ (on CelebA-Age). \todo{How? If there are no x-labels there should be no effect? this statement doees not explain why the performance is worse. It explains though why there is high variance.}

% But, interestingly as we saw earlier that \textit{MTA-F} even though always uses $ex_t$ for fairness update of $\theta_t$ does not suffer as negatively as \our\textit{-ex}. This showcases a drawback of \our~when trained $ex_t$. As \our~always uses one among $\mathcal{L}_t$ and $\mathcal{F}_t$ for any task $t$, any misinformed update on $\theta_t$ affects severely on the overall performance. \textit{MTA-F} on the other hand has less severe affect by using the summed loss $\mathcal{L}_t +\mathcal{F}_t$, with $\mathcal{L}_t$ being calculated on the entire set.    

%\todo{What is not shown here is why this happens, there is no space for the table iwth number of exclusive instances but at least this should be described in a short paragraph} 


==> l2tmcf.tex <==

\color{gray}
% While designing our algorithm we keep in note the above mentioned points. We lay our design goals as follows:
% \begin{itemize}
%     \item[i)] To keep the number of task weights required to be learned to $T$, where $T$ is number of tasks.
%     \item[ii)] To learn the optimal task weights automatically.
%     \item[iii)] To make sure that $\theta_t$ does not learns or reciprocates bias from data, and to have distinction between learning the $\theta_{sh}$ with learning $\theta_t$. 
% \end{itemize}
\color{black}

\color{gray}
% \subsection{A greedy loss function selection}
% \label{sec:ourGreedy}
% To achieve i) we reduce the fair-MTL problem (Eq.~\ref{eq:mtlfair_summed}) to a form of Eq.~\ref{eq:mtl}, which requires to optimize only one loss instead of two for each task at every training round. Now the simplest idea that may occur to implement this is by greedy selection of the loss function, i.e selecting the loss for a task  that has the highest computed scalar value as follows: 
% \begin{equation}\label{eq:greedy}
%     {argmin}_\theta \sum_t w_t \{\max \{\mathcal{L}_t(\theta,U), \mathcal{F}_t(\theta,S)\} \}
% \end{equation}
% Such a greedy setting may appear to be cost effective (same training complexity as any baseline MTL given in Eq.~\ref{eq:mtl}) and may work intuitively in terms of exploiting the loss surfaces. However, as seen in studies~\cite{foret2020sharpness}, loss surfaces can have steep minima. Now, for each single task we try to solve two different losses ($\mathcal{L}_t(\theta,U), \mathcal{F}_t(\theta,S)$) by taking a movement direction towards only one of the two loss gradients (say $\mathcal{L}_t(\theta,U)$) w.r.t $\theta$. In presence of a steep loss surface such movement may lead the model to converge to a sub-optimal region w.r.t to the other loss ($\mathcal{F}_t(\theta,S)$). 

% Recent development~\cite{fan2018learning2Teach,wu2018L2Tdynamic} has shown the advantages of informed decision making in presence of more than one loss. 
% Following that we base our work on a teacher student architecture~\cite{fan2018learning2Teach} where the MTL fair model is a student. The choice of which task specific loss function is best suited to learn for the student at any given training round for each of the task is decided by a teacher network $Q$. The teacher $Q$ for each task gives the instruction to learn a loss the student follows the instruction. The transformed learning problem is formulated as:
% \begin{equation}\label{eq:student_opti}
%     {argmin}_\theta \sum_t w_t \{argmax_{\alpha \in A(t)}Q(\alpha)\}
% \end{equation}
% where $A(t)=\{\mathcal{L}_t(\theta,U), \mathcal{F}_t(\theta,S)\}$.


% For goal ii) we take inspiration from~\cite{chen2018gradnorm}, and the learn the optimal task weights $w_t$ as parameters by optimizing Eq.~\ref{eq:grad_norm}. 
% For goal iii), whenever the student gets the signal from the teacher to learn from $\mathcal{F}_t$, we update $\theta_t$ with $\nabla_{\theta_t}\mathcal{F}_t$ instead of gradient info from Eq.~\ref{eq:student_opti}. Now we discuss the student and the teacher architecture in details. 
\color{black}
% \begin{algorithm}[!htbp]
% 	\caption{The L2T-FMT algorithm}
% 	\label{algo:l2t}
% 		\KwInput{A MTL dataset $D\in U\times S \times Y$ (see Section~\ref{sec:preliminaries})}
% 	\KwInit{Initialize student model  $\mathcal{M}$  parameters: $\theta=\theta_{sh}\times \theta_1\times\cdots\times\theta_T$ and 
% 	task weights: $w_t=\frac{1}{T}$\\
% 	Initialise teacher model $\mathcal{Q}$: parameters- $\theta^Q=\theta^Q_{sh}\times \theta^Q_1\times\cdots\times\theta^Q_T$ and environment weights  $\omega=\{\omega_t=\frac{1}{T}\}$
% 	}
% 	\begin{algorithmic}[1]
% 	    \State \textbf{Until} convergence \textbf{do}
% 	    \State \phantom{abv} \small$d=\{\argmax\limits_{\alpha \in \{\mathcal{L}_t,\mathcal{F}_t\}}Q(\theta_t,\alpha), \forall t\}$\normalsize \tcp{teacher decides the best loss to learn for student upon seeing $\theta_t$}
%         \State \phantom{abc} Call Algorithm~\ref{algo:stud} with input $(U,S,Y,d)$\tcp{Training $\mathcal{M}$}
%         %EIRINI: What is W?
%         %\State \phantom{abc} \textbf{for} $t=1,\cdots,T$ \textbf{do}
%         \State \phantom{abc} Evaluate $R=\{[\mathcal{R}(\mathcal{L}_t), \mathcal{R}(\mathcal{F}_t)]~\forall t\}$ using Eq.~\ref{eq:reward} \tcp{generate feedback for the teacher}
%         %\State \phantom{abc} \textbf{end for}
%         \State \phantom{abc} Call Algorithm~\ref{algo:teach} with input $(\{\mathcal{M}(t)\}, \{\theta_t\},R, A)$ \tcp{Training $Q$}
% 	\end{algorithmic}%}
% 	\KwOutput{$\mathcal{M}$ with learned parameters $\theta=\theta_{sh}\times \theta_1\times\cdots\times\theta_T$}
% \end{algorithm}









==> old_per_task.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/fair_pums.png}
         \caption{ACS-PUMS}\label{fig:per_pums}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/fair_gender.png}
         \caption{CelebA-Gender}\label{fig:per_gen}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
     \includegraphics[width=\linewidth]{Figures/fair_age.png}
         \caption{CelebA-Age}\label{fig:per_age}
    \end{subfigure}
    \caption{Per-task fairness evaluation in all datasets (lower values are better).}
    \label{fig:expPerTaskFairness}
\end{figure*}


\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/acc_pums.png}
         \caption{ACS-PUMS}\label{fig:per_pums_acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/acc_gender.png}
         \caption{CelebA-Gender}\label{fig:per_gen_acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
     \includegraphics[width=\linewidth]{Figures/acc_age.png}
         \caption{CelebA-Age}\label{fig:per_age_acc}
    \end{subfigure}
    \caption{Per-task accuracy evaluation in all datasets (higher values are better).}
    \label{fig:expPerTaskAccuracy}
\end{figure*}


%\subsubsection{Per-task Fairness Analysis }
\phantom{ddd}

\noindent\textbf{Per-task performance: ACS-PUMS dataset.}
The per-task fairness and accuracy results are shown in  Fig~\ref{fig:per_pums} and Fig~\ref{fig:per_pums_acc}, respectively.
W.r.t. to fairness, we notice (Fig~\ref{fig:per_pums}) that \our~outperforms the competitors in \textbf{3 out of 5} tasks (1, 3, and 5) achieving the lowest EO$_{viol}$ scores  ($<0.01$)
and it even outperforms the respective STL models in two tasks (3, and 5). 
From Fig~\ref{fig:per_pums_acc} we see that \our~maintains a high accuracy ($>0.72$) in all the tasks and outperforms the competitors in \textbf{2 out of 5} tasks (2, and 3).

Considering the combined fairness and accuracy performance, we see that \our scores first in task 1  (\textit{Employment status} prediction) with top accuracy of 0.98 and lowest EO$_{viol}$ score of 0.01. Note that all methods perform well in Task 1 w.r.t. accuracy (low spread) but they differ w.r.t. fairness performance (large spread).
Similarly, for task 3 (\textit{Health Insurance status} prediction), \our has the lowest  EO$_{viol}$ and the highest accuracy after STL. \textit{MTA-F} performs poorly in this task with the lowest accuracy among the compared methods and the highest discrimination.
In overall, \textit{MTA-F} performs decently w.r.t. fairness (it even outperforms \our~in fairness for task 4  (\textit{Work Travel time} prediction)). However, it has the lowest accuracy for task 4 and in general, its accuracy is the lowest for most of the tasks (3, 4 and 5).


\color{green}
\todo{A natural question here is whether the impact of the batch size has been properly evaluated. @Arjun: to discuss}
Our usage of a very large batch size (c.f Sec.\ref{sec:repro}) lets us in our experiment avoid the problem highlighted in Fig~\ref{fig:labels_exclusive} for the ACS-PUMS dataset for MTA-F.  
\color{black}

The \textit{Vanilla MTL} despite having no fairness treatment, outperforms MTA-F in fairness, producing the second worst AREO score (see Table~\ref{tab:exp}), 
with the highest EO$_{viol}$ scores in 2 out 5 tasks (1, and 2), but it is also the most accurate model overall with the best accuracy scores in tasks 3 and 4 (and highest ARA score, see Table~\ref{tab:exp}). 

The \textit{G-FMT} equals the EO$_{viol}$ scores of \our~in 4 out of 5 tasks, henceforth comes out as the second best fair classifier (also reflected in the second best AREO score, in Table~\ref{tab:exp}.

\noindent \textbf{Per-task performance: CelebA-Gender dataset.} 
The superior performance of our  \our~is shown in Fig~\ref{fig:per_gen_acc} (for fairness) and Fig~\ref{fig:per_gen} (for accuracy).
 \our~outperforms the competitors in accuracy in \textbf{10 out of 17} tasks, and in fairness in \textbf{15 out of 17} tasks. \our~even outperforms the respective \textit{STL} models 3 times both in accuracy and fairness for tasks 3 (\textit{Bangs}), 8 (\textit{Bushy Eyebrows}), and 11 (\textit{Narrow Eyes}). 
 
%occasions by achieving the lowest  EO$_{viol}$ scores of $\leq0.02$  in tasks 2,7,8,9,10,14,17 and  $<0.05$ in all the other tasks.
\color{red}
\textit{MTA-F}'s relative positioning among the competitors  improved overall in the CelebA-Gender in comparison that in ACS-PUMS. \textit{MTA-F} achieved the second best ARA and the third best AREO score. However, looking carefully in Fig~\ref{fig:per_gen} and Fig~\ref{fig:per_gen_acc} we notice that it has very high EO$_{viol}$ scores in task 11 while having second lowest accuracy. This outcome highly hampers its overall relative average (AREO and ARA). 
\color{black}
On careful analysis of the data we see that for the task 11 (\textit{Narrow Eyes}) there approx. 40 task exclusive label per batch (c.f~Sec.\ref{sec:repro}) of training data. The gradient update of the task exclusive layers which depends on the computation of fairness loss from these task exclusive labels becomes very unstable due the lack of data. This incident particularly highlights the problem with the method which can make the fairness outcome very unstable in presence of large number of tasks. However, the problem do not persists in other tasks in the data. Intuitively, this may be because the exclusive labels in them are almost non-existent, which incidentally doesn't let the method to hinder the task exclusive layer with unstable gradient info. 
The \textit{G-FMT} emerges as the second best fair method with second lowest  EO$_{viol}$ scores in 14 out of 17 tasks.However, the accuracy of the model relative to the other competitors is poor with the lowest accuracy score in 8
%(task 2, 3, 4, 5, 7, 12, 13, and 17) 
out of 17 tasks, does contributing towards its lowest ARA score (see Table~\ref{tab:exp}).

The \textit{Vanilla MTL} has the most unfair outcomes in  11 out of 17 tasks with highest EO$_{viol}$ scores which contributes to its overall highest AREO scores as seen in Table~\ref{tab:exp}. The accuracy of the model apart from a single task (task 8) never excels the other competitors and in 7 out 17 tasks it produces either the lowest (task 10 and 16) or the second lowest (tasks 2, 7, 12, 13 , and 17) accuracy scores.  


%\our~emerges as the most fair classifier in both the Visual data experiments, outperforming all the MTL competitors on Visual 1 data in \textbf{15 out of 17} tasks, On the Visual 2 data also \our~outperforms the MTL competitors in \textbf{15 out of 31} tasks and bettering the STLs in 12 occasions by consistantly achieving low EO$_{viol}$ scores of $<0.04$ in all the tasks, with $0.02$ in 17 different tasks. The outcomes establishes the genralizability of the method under large number of multi-tasks.
\noindent \textbf{Per-task performance: CelebA-Age dataset.}
\color{red}
Fig~\ref{fig:per_age_acc} and Fig~\ref{fig:per_age} depicts the generalizability of \our~in presence of large number of tasks in the CelebA-Age data, outperforming the MTL competitors on \textbf{14 out of 31} tasks in accuracy \textbf{15 out of 31} tasks in fairness. \our~betters the STLs in 12 occasions on fairness by consistently achieving low EO$_{viol}$ scores. 
%of $<0.04$ in all the tasks, with $<0.02$ in 17 different tasks. 
Specifically in task 12 (\textit{Heavy Makeup}) and 22 (\textit{Sideburns}), \our~achieved the best EO$_{viol}$ score of \textbf{0.01} and \textbf{0.03}, with accuracy score $>0.9$.

\textit{MTA-F} performed decently in the CelebA-Age, even outperforming the other competitors in 6 out 31 tasks on fairness, but in none of the task it outperformed the others in accuracy. Again, by analysing the data a similar conclusion as above in CelebA-Gender results can be drawn for MTA-F, as in presence of large number (31) of tasks, the task exclusive labels are non-existent. 

For \textit{G-FMT} in Table~\ref{tab:exp} we see that it had very similar ARA and AREO score as that of \textit{MTA-F}. However, from Fig~\ref{fig:per_age_acc} and Fig~\ref{fig:per_age} we see that \textit{G-FMT} in none of task outperformed the competitors in fairness, and in 11 out of 31 tasks it have the lowest accuracy, thus may be argued as a less preferable choice over \textit{MTA-F} in the CelebA-Age.  
\color{black}

The \textit{vanilla MTL} is again the most unfair classifier with highest EO$_{viol}$ scores in 22 out of 31 tasks. The G-FMT owing to its greedy characteristics, which gives an added advantage to the method of producing decent performance while saving on time complexity, has the second best fairness outcome in 13 out of 31 tasks.


\noindent\textbf{Summary:} 
Overall, the experiments show that \our~consistently achieves low EO$_{viol}$ scores in varying data types and number of tasks. 
%The outcomes establishes the genralizability of the method under large number of multi-tasks. 
The \textit{MTA-F} method is very unstable under large number of tasks, probably because its gradient update of the task exclusive layers becomes very unstable due to lack of task exclusive labels.  
The \textit{vanilla MTL} as expected without any fairness treatment, emerges to be most unfair classifier overall. The greedy approach \textit{G-FMT} even though never able to outperform all the other competitors, it is often the second best  competitor, owing to the natural comprehension of the greedy characteristic of delivering cost-effective of decent performances. The outcome also portrays that choosing one among fair and empirical loss for each task, is sufficient to produce a fair MTL classifier instead of optimizing for both together for each task.


==> todos.tex <==
EO or EO_{viol}: check everywhere

Table 2: looks bad, it can occupy the full width.
use a conventional layout, e.g., https://i.stack.imgur.com/h996K.png

Figure 5.a, is task 11 also the worse task for vanilla-MTL? Can you check? 11 is the worse for MTA-F.
== it is task 11 the worst for both methods

In experiments we mention task 1 ... 44, please add those IDs also in the appendix


Whenever referring to a figure please use Fig.  (with the dot)

